Graphical Perception in Animated Bar Charts

Interactive visual applications create animations that encode changes in the data. For example, cross-filtering dynamically updates linked visualizations based on the user's continuous brushing actions. The animated effects resulting from these interactions depends both on how interaction (e.g., brushing speed) controls properties of the animation such as frame rate, as well as how the data that is being explored dictates the data encoded in the animation. Past work has found that frame rate matters to general perception, however a critical question is which of these animation and data properties affects the perceptual accuracy of judgement tasks, and to what extent. Although graphical perception has been well studied for static data visualizations, it is ripe for exploration in the animated setting. We designed two animated judgment tasks of a target bar in an animated bar chart and empirically evaluate the effects of 2 animations properties - highlighting of the target bar and frame rate - as well as 3 data properties that affect the target bar's value throughout the animation. In short, we find that the rate and timing of animation changes is easier detected in larger values; that encodings such as color are easier to detect than shapes; and that timing is important - earlier changes were harder to perceive as compared to later changes in the animation. Our results are an initial step to understanding perceptual accuracy for animated data visualizations, both for presentations and ultimately as part of interactive applications.

==> content/exp.tex <==
\section{Experimental Methodology}
We ran several perceptual studies, described in the
subsequent sections, that: 
\begin{enumerate}
\item replicate prior static perceptual studies 
\item measure judgment tasks in non-approximated animated data visualizations, and 
\item measure judgment of animated data visualizations in the presence of various approximation techniques. 
\end{enumerate}

This section describes the common features and protocols
that we used across our studies.
When possible, we used analysis procedures similar to previous 
studies~\cite{cleveland1984graphical, heer2010crowdsourcing, talbot2014}.

\ewu{justify animation}

We employ a within-subjects format and use a custom multi-task interface to manage the multiple judgment tasks in each human intelligence task (HIT).  
Each experiment is a separate HIT deployed on the Amazon Mechanical Turk~\cite{mturk} marketplace and we pay subjects using bonuses. 
Similar to previous studies, subjects must pass several qualification and training tasks before participating in an experiment.  
Qualification tasks are drastically simplified versions of tasks to ensure worker comprehension of the task interface and are specific to the experiment; we reject subjects that fail the qualification.
Training tasks are in the exact format as the experiment tasks, however we show the correct
answer upon submission and do not reject subjects to avoid bias.  
% The training tasks do not use rounded target bar values to avoid bias towards rounded or evenly spaced answers~\cite{talbot2014}.
The judgment tasks within a HIT are shown in random order. Along with task
responses, we record auxiliary information such as the browser,
display size, and response time.

We pay $\$0.05$ for each task (including qualification and training tasks). 
To encourage subjects to finish all of the judgment tasks in a HIT, we offer a $\$1.00$ bonus upon completion of the full HIT.
We submitted a total of $1530$ HITs, of which $715$ were completed, and $575$ ($41,623$ judgments) were used in analysis.
Due to the unexplored nature of this area of research, we are forced to make a trade off between practical budget limitations and coverage of experiments -- we chose to prioritize experimental coverage.
For this reason, many of our experiments reflect sample sizes from a modest number of assignments due to many disqualified workers.
Despite this, confidence intervals are kept relatively tight in many experiments, and we are still able to draw insights from the results.
% \ewu{check the above para -- i focused on stating our case, but not sounding weak -- arnab}
% \ewu{the math seems to be (41623*0.05)+715 = \$2796 -- can you check? Do we want to mention that?}

\if{0}
Whenever possible, we used analysis procedures similar to previous 
related studies~\cite{cleveland1984graphical, heer2010crowdsourcing, talbot2014}.
We discard results from workers with incomplete experiment tasks,
spammers whose judgments vary by less than $15$~(true values vary from $18$ to $85$), and 
workers whose correlation with the true results are below a threshold (defined in each section)~\cite{talbot2014}.
\fi

% Following prior studies~\cite{cleveland1984graphical,heer2010crowdsourcing,talbot2014}, we use a log absolute error measure of accuracy: 




==> content/macro.tex <==
% From http://tex.stackexchange.com/questions/32182/using-indentation-to-automatically-begin-and-end-itemize-environments

\def\+{+}

\makeatletter
\catcode`\ =12\let\@nl@space= \catcode`\ =10
\newcount\@nl@rlevel
\newcount\@nl@llevel
\@nl@llevel=-1

\def\@nl{%
  \catcode`\ =12
  \global\@nl@rlevel=0
  \futurelet\@nl@store\@nl@%
}
\def\@nl@gobble#1{\futurelet\@nl@store\@nl@}
\def\@nl@enditemize{
  \ifnum\the\@nl@rlevel<\the\@nl@llevel%
    \end{itemize}%
    \egroup%
    \expandafter\@nl@enditemize%
  \else%
    \ifnum\the\@nl@rlevel=\the\@nl@llevel\else%
       \errmessage{Error: inconsistent identation}
    \fi%
  \fi%
}
\def\@nl@{%
  \ifx\@nl@store\@nl@space%
    \global\advance\@nl@rlevel by 1
    \expandafter\@nl@gobble%
  \else%
    \catcode`\ =10
    \ifx\@nl@store+%
      \ifnum\the\@nl@rlevel>\the\@nl@llevel%
        \bgroup%
        \@nl@llevel=\the\@nl@rlevel
        \begin{itemize}%
      \fi%
      \@nl@enditemize%
      \item \expandafter\expandafter\expandafter\@gobble%
    \else%
      \ifx\@nl@store\@nl%
        \global\@nl@rlevel=-1\relax\@nl@enditemize\par
      \else\space\fi%
    \fi%
  \fi%
}

\catcode`\^^M=\active%
\AtBeginDocument{%
  \catcode`\^^M=\active%
  \let^^M=\@nl%
}%
\catcode`\^^M=5
\makeatother

